Block Distributed Majorize-Minimize Memory Gradient Algorithm and its application to 3D image restoration

Modern 3D image recovery problems require powerful optimization frameworks to handle high dimensionality while providing reliable numerical solutions in a reasonable time. In this perspective, asynchronous parallel optimization algorithms have received an increasing attention by overcoming memory limitation issues and communication bottlenecks. In this work, we propose a block distributed Majorize-Minorize Memory Gradient (BD3MG) optimization algorithm for solving large scale non-convex differentiable optimization problems. Assuming a distributed memory environment, the algorithm casts the efficient 3MG scheme into smaller dimension subproblems where blocks of variables are addressed in an asynchronous manner. Convergence of the sequence built by the proposed BD3MG method is established under mild assumptions. Application to the restoration of 3D images degraded by a depth-variant blur shows that our method yields significant computational time reduction compared to several synchronous and asynchronous competitors, while exhibiting great scalability potential.

==> BD3MG IEEE (Version 4834)/Implementation.tex <==
% !TEX root = icip2016.tex

\section{Application to 3D image deblurring}

\subsection{Model and objective function}
We consider the restoration of a 3D microscopic volume $\overline{x}$ of size $N = N_{\mathsf{X}} \times N_{\mathsf{Y}} \times N_{\mathsf{Z}}$, given a degraded observation $y$, altered by a depth-variant blur operator $H$ and an additive white noise $b$: 
\begin{equation}\label{eq:model}
y = H \overline{x} + b.
\end{equation}
The associated inverse problem can be solved efficiently by minimizing a least squares penalization penalized by a smooth 3D regularization function. Specifically, $f$ takes the form:
\begin{equation}\label{eq_crit}
\forall x \in \mathbb{R}^N, \quad f(x) = \sum_{s=1}^4 f_{s} (L_sx)
\end{equation} with $f_1 \circ L_1 = \frac{1}{2} \| H \cdot - y\|^2$, $f_2 \circ L_2 = \eta\, d^2_{[x_{\min},x_{\max}]^N}$,  $f_3 \circ L_3 = \lambda \sum_{n=1}^N \sqrt{ \left([V^{\mathsf{X}} \cdot]_n\right)^2 + \left( [V^{\mathsf{Y}} \cdot]_n\right)^2 + \delta^2}$, and $f_4 \circ L_4 = \kappa \| V^{\mathsf{Z}} \cdot \|^2$. 
% :
% \begin{itemize}
%     \small
% 	\item $L_1 = H$, $f_1 = \frac{1}{2} \| \cdot - y\|^2$,  
% 	\item $L_2 = \mathbb{I}_N$, $f_2 = \eta\, d^2_{[x_{\min},x_{\max}]^N}$
%     \item $L_3 = [(V^{\mathsf{X}})^\top (V^{\mathsf{Y}})^\top]^\top$, \\$f_3(L_3 x) = \lambda \sum_{n=1}^N \sqrt{ \left([V^{\mathsf{X}} x]_n\right)^2 + \left( [V^{\mathsf{Y}} x]_n\right)^2 + \delta^2}$, 
%     \item $L_4 = V^{\mathsf{Z}}$, $f_4 = \kappa \| \cdot \|^2$
% \end{itemize}
% \vspace{0.3cm}
Hereabove, $V^{\mathsf{X}} \in \eR^{N \times N}$, $V^{\mathsf{Y}} \in \eR^{N \times N}$, $V^{\mathsf{Z}} \in \eR^{N \times N}$ state for discrete gradient operators along the three directions of the volume, $x_{\min}$ (resp $x_{\max}$) $\in \eR$ are minimal (resp. maximal) bounds on the sought intensity values and $d_E$ is the Euclidian distance to set $E$. Function $f$ satisfies Ass.~\ref{Ass:A} as a combination of squared distances and discretized total-variation distances.  If not specified otherwise, the majorizing matrices for $f$ will be constructed following the strategy in \cite{Chouzenoux_2013}, ensuring the fulfillment of Ass.~\ref{Ass:C}. The convolution operator $H$ simulates a depth-varying 3D Gaussian blur. For each depth $z \in \{1,\ldots, N_{\mathsf{Z}}\}$, the blur kernel is characterized by different variance and rotation parameters whose values are taken as random realizations of uniform distributions. The depth-variant structure of the blur model motivates us to split the vector $x$ along the dimension $\mathsf{Z}$, assigning computing agents (i.e. workers) to one (or several) selected slice(s) of the 3D volume. For the sake of simplicity, a sequential ordering is used, for the selection rule of the processed blocks, hence Ass.~\ref{Ass:B} is fulfilled. Furthermore, the same strategy as in \cite{7532949} is employed to control the memory usage during communications master/worker. All algorithms are initialized with $x^0 \in \mathbb{R}^N$ whose entries are uniformly sampled in $[0,\max(y)]$. Parameters $\lambda, \eta, \delta, \kappa>0$ will be tuned manually, for both presented examples, so as to maximize the Signal-to-Noise Ratio (SNR) of the restored volume. Two microscopic images, namely \texttt{FlyBrain} and \texttt{Aneurysm} will be considered. Example of restoration results are presented in Fig.~\ref{fig:visual}.

%  Two microscopic images, namely \texttt{FlyBrain} and \texttt{Aneurysm}, with respective size $N = 256 \times 256 \times 24$ and $N = 256 \times 256 \times 79$, respectively, will be considered. 


% Parameters $\lambda, \eta, \delta, \kappa \in [0,+\infty)^4$ will be tuned manually, for both presented examples, so as to maximize the Signal-to-Noise Ratio (SNR) of the restored volume.

% The matrices $\mathcal{A}$ are constructed similarly to \cite{Chouzenoux15gretsi} . For $\overline{x}$, the 3D microscopic image \texttt{FlyBrain}\footnote{http://imagej.nih.gov/ij/plugins/3d$-$viewer/} and \texttt{Aneurysm} were considered with truncated size $N = 256 \times 256 \times 24$. The convolution operator $H$ models a depth-varying 3D Gaussian blur. For each depth $z \in \{1,\ldots, N_{\mathsf{Z}}\}$, the blur kernel of size $11 \times 11 \times 21$ is characterized by different variance and rotation parameters $(\sigma_{\mathsf{X}}(z),\sigma_{\mathsf{Y}}(z),\sigma_{\mathsf{Z}}(z),\varphi_{\mathsf{Y}}(z),\varphi_{\mathsf{Z}}(z))$, as described in \cite{Wirjadi05} whose values are independent realizations of a uniform distribution. A white Gaussian noise with standard deviation $0.04$ is then added to the blurred volume. We tune the parameters $\lambda, \eta, \delta, \kappa$ in $[0,+\infty[$ so as to maximize the Signal-to-Noise Ratio (SNR) of the restored volume. 


% One core is used as the Master to perform the main loop while all the $C = \overline{C}-1$ other workers are computing asynchronously their update depending only on their communication with the Master. We split the coordinates blocks along the z-axis so as to balance the trade-off between saturation of Master queue and significance of working agents updates. The experiment was performed using \textit{Python} and its built-in \textit{Multiprocessing} library on an Intel® Xeon(R) W-2135 CPU with 12 cores clocked at 3.70GHz.
\subsection{Ablation study and comparative analysis}

In order to measure the performance improvement allowed by BD3MG, we conducted an ``ablation study'', that consists in removing some/all acceleration features of our algorithm, namely asynchrony, subspace line-search and MM scaling. We then obtain, in addition to BD3MG, four parallel/distributed optimization algorithms that we detail hereafter. The \emph{asynchronous gradient descent} (Async-GD) corresponds to the algorithm from \cite{niu2011hogwild}, obtained by limiting the subspace to the sole gradient descent direction $\mathcal{D}_{(\mathcal{S})}(x) = - \nabla_{(\mathcal{S})}f(x)$ and by setting $\mathcal{A}_{(\mathcal{S})} = \mathcal{L} \, \mathrm{Id}_{|\mathcal{S}|}$, with $\mathcal{L}$ the Lipschitz constant of $\nabla f$. The \emph{asynchronous conjugate gradient} algorithm (Async-CG) identifies with our BD3MG method when using the basic MM metric $\mathcal{A}_{(\mathcal{S})} = \mathcal{L} \, \mathrm{Id}_{|\mathcal{S}|}$. The resulting algorithm can be viewed as a distributed version of the nonlinear conjugate gradient method, with closed form stepsize from \cite{Labat2008}. The \emph{asynchronous MM algorithm} (Async-MM) is obtained by removing the subspace acceleration strategy in BD3MG, so that $d'_{S} = - \mathcal{A}_{(\mathcal{S})}(x)^{-1} \nabla_{(\mathcal{S})}f(x)$ in the Worker loop. The latter inversion is performed with linear biconjugate gradient solver. Async-MM can be interpreted as a distributed implementation of a half-quadratic algorithm \cite{Allain2006}. Finally, \emph{block parallel 3MG algorithm} (BP3MG) is the method we originally proposed in  \cite{7532949}, where blocks updates are assumed to be computed at the same time without any communication delay. The names and characteristics of the resulting five tested methods are summarized in Tab.~\ref{tab:optisetup}.

\begin{table}[h]
  \centering
  \small
  \begin{tabular}{|c||ccc|} 
    \hline
    Name & Asynchrony & Memory & MM scaling \\
    \hline\hline
    Async-GD & \checkmark  & \xmark & \xmark  \\
    \hline
    Async-CG & \checkmark & \checkmark & \xmark   \\
    \hline
    Async-MM & \checkmark & \xmark & \checkmark \\
    \hline
    BP3MG & \xmark & \checkmark & \checkmark \\
    \hline
    \hline
    BD3MG & \checkmark & \checkmark & \checkmark\\
    \hline
  \end{tabular}
   \caption{Algorithmic features of the compared approaches.}
  \label{tab:optisetup}
\end{table} 
\vspace{-0.6cm}
\begin{figure}[h]
%\setlength{\belowcaptionskip}{-15pt}
\includegraphics[width=8.5cm]{comparaison_Error_SNR.png}
\caption{Evolution of SNR in dB (left) and relative distance to solution $\|x^k-x^{*}\|/\|x^{*}\|$ (right) along time (in seconds) for \texttt{FlyBrain} restoration. Results are averaged over ten noise realizations.}
\label{fig:comp}
\end{figure}

%
% \begin{table}[ht]
%   \centering
%   \begin{tabular}{|c||cc|} 
%     \hline
%     Version & \textbf{SNR} (at 1e3 sec) & \textbf{Time} ($\|x-x^{*}\|<\epsilon\|x^{*}\|$) \\
%     \hline\hline
%     Async-BGD & 14.210 \pm 0.002 & 896.2 \pm 8.5  \\
%     \hline
%     Async-ABGD & 14.297 \pm 0.003 & 802.5 \pm 18.8   \\
%     \hline
%     Async-CGD & 3.665 \pm 0.021 & - \\
%     \hline
%     BP3MG & 14.331 \pm 0.001 & 988.7 \pm 14.0    \\
%     \hline
%     \textbf{BD3MG} & \textbf{14.335} \pm \textbf{0.002}& \textbf{346.5}\pm\textbf{15.3}\\
%     \hline
%   \end{tabular}
%   \caption{Comparison of \texttt{FlyBrain} reconstruction results for the 5 different optimisation strategies.}
%   \label{tab:resultable}
% \end{table}
%

We perform our comparative analysis, using the microscopic image  \texttt{FlyBrain} with size $N = 256 \times 256 \times 24$. It is degraded by depth-variant blur kernels of size $11\times 11 \times 21$, and a zero-mean white Gaussian noise with standard deviation $0.04$. The results are averaged over ten noise realizations, and the initial signal to noise ratio is around $11.6$ dB. Fig.~\ref{fig:comp} illustrates the evolution of the SNR of the restored image along time in seconds, for each method, for experiments performed using Python 3, running an Intel® Xeon(R) W-2135 CPU with 12 cores clocked at 3.70GHz. We also display the relative distance to the solution $x^*$, computed after a large number of iterations (typically, $10^4$), characterized by an average SNR of $14.33$ dB. One can see that the proposed BD3MG method clearly outperforms the others in terms of time to reach close-to-optimal solution. Async-MM led to the slowest convergence, as it requires linear system inversion at each iteration. The superiority of Async-CG over Async-GD illustrates the benefits for including the memory term within the subspace. Finally, BD3MG reaches convergence faster than its synchronous counterpart, BP3MG, probably thanks to the removal of the locking conditions in the Master loop. 
% The second best option is Async-CG, which shows the great interest 
% \cred{All three discussed algorithmic features prove to significantly accelerate convergence in this experiment as the MM scheme without Memory gradient takes too much time per iteration (BD3MG vs Asynch-MM) while the trade-off between reduction of agents idle time and error due to delayed information is favorable to the asynchronous version (BD3MG vs BP3MG).}


\begin{figure}[h]
    \centering
\begin{tabular}{@{}c@{}}
 \includegraphics[width=8cm]{flybrainrec.png}\\
    \includegraphics[width=8cm]{aneyrismrec.png}
\end{tabular}
    \caption{Comparison between original (\textbf{left}), degraded (\textbf{middle}) and restored (\textbf{right}) slices ($z=10$) of \texttt{FlyBrain} and \texttt{Aneurysm}.}
    \label{fig:visual}
\end{figure}

% \begin{figure}[h]
%     \centering
% \begin{tabular}{@{}c@{}c@{}c@{}}
%  \includegraphics[width=2.8cm]{Fly_I_z10.png}&
%   \includegraphics[width=2.8cm]{Fly_Iblurnoisy_z10.png}&
%   \includegraphics[width=2.8cm]{Fly_Irec_z10.png}\\
%   \includegraphics[width=2.8cm]{Fly_I_z20.png}&
%   \includegraphics[width=2.8cm]{Fly_Iblurnoisy_z20.png}&
%   \includegraphics[width=2.8cm]{Fly_Irec_z20.png} 
% \end{tabular}
%     \caption{Comparison between original (\textbf{left}), degraded (\textbf{middle}) and restored (\textbf{right}) slides of \texttt{FlyBrain} at altitude $z=10$ and $z=20$.}
%     \label{fig:visual}
% \end{figure}

% \begin{figure}[h]
%     \setlength{\belowcaptionskip}{-15pt}
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \includegraphics[width=8.5cm]{flybrainrec.png}
% %\vspace{-0.4cm}
%     \end{subfigure}%
    
%     \begin{subfigure}[t]{0.5\textwidth}
%         \includegraphics[width=8.5cm]{aneyrismrec.png}
%     \end{subfigure}
%     \caption{Comparison between original (\textbf{left}), degraded (\textbf{middle}) and restored (\textbf{right}) versions of \texttt{FlyBrain} (first row) and \texttt{Aneurysm} (second row). The images corresponds to 2D horizontal slice at altitude $z=10$ for both 3D volumes.}
%     \label{fig:visual}
% \end{figure}

% We synthetically tested different computing environment in order to qualify the value of the asynchronous version, by adding stochastic delay in the computing loop of the computing agents. The three following scenarii were tested:
% \begin{itemize}
%     \item \textbf{I} : One core of the pool of "workers" is consistently affected by a delay that follows a uniform distribution $\mathcal{U}([0,1])$ (in sec.). The other cores are not affected by any delay. 
%     \item \textbf{II} : Two "worker" cores are not affected by any delay while the others 9 agents are set in the following fashion:
%         \begin{itemize}
%             \item 3 cores hold a delay following a uniform distribution $\mathcal{U}([0,1])$.
%             \item 3 cores hold a delay following a uniform distribution $\mathcal{U}([0,0.5])$.
%             \item 3 cores hold a delay following a uniform distribution $\mathcal{U}([0,.25])$.
%         \end{itemize}
%     \item \textbf{III} : All the "worker" cores are consistently affected by a delay that follows a uniform distribution $\mathcal{U}([0,1])$.
% \end{itemize}
% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=6.5cm]{comparaison_BD_vs_BP.png}
% %\vspace{-0.4cm}
%         \caption{Value of criteria as a function of time during optimization for \texttt{FlyBrain} reconstruction}
%         \label{fig:acceler}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=5cm]{idle_time.png}
%         \caption{Idle time of CPUs (as a percentage of total time) for the three different settings. (Red is BP3MG and Green is BD3MG)}
%         \label{fig:idle}
%     \end{subfigure}
% \end{figure}
% \noindent The results of our experiment is presented in table (\ref{tab:ecarts}), graph (\ref{fig:acceler}) and (\ref{fig:idle}). In all three scenarii, \textbf{BD3MG} outperfoms its synchronous version in terms of time while reaching a similar value criterion and SNR. Even though the descent scheme is not enforced as discussed in section (\ref{sec:preliminaries}), the criteria descent is quicker due to accelerated iterations of the workers and a more efficient handling of workload as shown in figure (\ref{fig:idle}) where CPU idle time is consistently lower. We note that in an asymmetric setting such as (I), BD3MG prooved to be particurlay efficient in reducing the deadlock for "quick" workers.
% \vspace{-0.6cm}
% \begin{figure}[htb!]
% \centering
% \includegraphics[width=10cm]{comparaison_BD_vs_BP.png}
% %\vspace{-0.4cm}
% \caption{Value of criteria as a function of time during optimization for \texttt{FlyBrain} reconstruction}
% \label{fig:acceler}
% \end{figure}
% \begin{figure}[htb!]
% \centering
% \includegraphics[width=8cm]{idle_time.png}
% %\vspace{-0.4cm}
% \caption{Idle time of CPUs (as a percentage of total time) on the 12-cores machine used in experience (1) for the three different types of settings in the reconstruction of \texttt{FlyBrain}.(Red is BP3MG and Green is BD3MG). }
% \label{fig:acceler}
% \end{figure}
% \subsection{Acceleration}

\subsection{Linear Speedup}

In order to assess the scalability of the BD3MG algorithm, we further analysed the speed-up of the optimization process when a High Parallel Computing computer is being used. Namely, we ran BD3MG and BP3MG on an Intel Xeon CPU 6148 with up to 80 physical cores at 2.4 GHz (Skylake) and 1.5 Tio of RAM. Image \texttt{Aneurysm} with size $N = 155 \times 154 \times 79$ is degraded by blur kernels of size to $5 \times 5 \times 11$, and noise standard deviation of $0.04$, so that the initial SNR is $6.44$ dB, while the restored SNR is $11.92$ dB. Fig.~\ref{fig:speedup} presents the acceleration ratio between the required computation time for two cores (i.e. one Master and one Worker) versus the computation time when activating from 10 to 80 cores, for reaching the stopping criterion $\|x^{k+1}-x^k\| \leq 10^{-6} \|x^k\|$. This illustrates the great potential of scalability of the proposed algorithm. Asynchronicity of BD3MG allows to improve the speed-up, in comparison to the one exhibited by BP3MG \cite{7532949}. Finally, as the number of core increases, a mild saturation effect is observed (in
agreement with Amdahl’s law \cite{Amdahl}).

\begin{figure}[htb!]
\setlength{\belowcaptionskip}{-10pt}
\centering
\includegraphics[width=5cm]{Acceleration2.png}
%\vspace{-0.4cm}
\caption{Speed-up ratio for BD3MG (blue) and BP3MG (red), with respect to the number of active cores for the restoration of \texttt{Aneurysm}.}
\label{fig:speedup}
\end{figure}

% % Fig.~\ref{fig:resim} displays some examples of original, degraded and restored slices, for two slices of \texttt{FlyBrain}. In Fig.~\ref{fig:acceler}, we plot, for different values of the number of active cores $\overline{C}$, the ratio between the required computation time for one core versus the actual computational time, for reaching the stopping criterion $\|x_k - x_{k-1}\| \leq 10^{-3} \| x_k \|$. The computations were performed using HPC resources from the “Mésocentre” computing center of CentraleSupélec and École Normale Supérieure Paris-Saclay supported by CNRS and Région Île-de-France (http://mesocentre.centralesupelec.fr/). The hardware used is an Intel Xeon CPU 6148 with 80 physical cores at 2.4 GHz (Skylake) and 1.5 Tio of RAM. The result of a linear fitting illustrates the great potential of parallelization of the proposed algorithm. 
% \begin{figure}[h!]
% \begin{center}
% \begin{tabular}{@{}c@{}c@{}c@{}}
% \includegraphics[width=3cm]{I_256_48_z6} & \includegraphics[width=3cm]{Iblurnoisy_256_48_z6} & \includegraphics[width=3cm]{Irec_256_48_z6}\\
% \includegraphics[width=3cm]{I_256_48_z18} & \includegraphics[width=3cm]{Iblurnoisy_256_48_z18} & \includegraphics[width=3cm]{Irec_256_48_z18}\\
% %\includegraphics[width=3cm]{I2_370_36_z20} & \includegraphics[width=3cm]{I2blurnoisy_370_36_z20} & \includegraphics[width=3cm]{I2rec_370_36_z20}\\
% %\includegraphics[width=3cm]{I2_370_36_z29} & \includegraphics[width=3cm]{I2blurnoisy_370_36_z29} & \includegraphics[width=3cm]{I2rec_370_36_z29}
% \end{tabular}
% \end{center}
% %\vspace{-0.7cm}
% \caption{Original (left), degraded (middle) and restored (right) images corresponding to slices $z = 6$ (top) and $z = 18$ (bottom) of the 3D volume \texttt{FlyBrain}.}
% \label{fig:resim}
% \end{figure}
% %\begin{figure}[h!]
% %\begin{center}
% %\begin{tabular}{@{}c@{}c@{}}
% %\includegraphics[width=4cm]{I_256_48_z6} & \includegraphics[width=4cm]{I_256_48_z18} \\
% %\includegraphics[width=4cm]{Iblurnoisy_256_48_z6} & \includegraphics[width=4cm]{Iblurnoisy_256_48_z18} \\
% %\includegraphics[width=4cm]{Irec_256_48_z6} & \includegraphics[width=4cm]{Irec_256_48_z18} \\
% %\end{tabular}
% %\end{center}
% %\vspace{-0.7cm}
% %\caption{\small Original (left), degraded (middle) and restored (right) images corresponding to slices $z = 6$ (top) and $z = 18$ (bottom) of the 3D volume.}
% %\label{fig:resim}
% %\end{figure}
% \begin{figure}[h!]
% \centering
% \begin{tabular}{@{}cc@{}}
% \includegraphics[width=4cm,height=3.8cm]{acceleration} & \includegraphics[width=4cm,height=3.8cm]{acceleration_tube}
% \end{tabular}
% %\vspace{-0.4cm}
% \caption{Ratio between the computation time for one core and the computation time for $\overline{C}$ cores (crosses) with linear fitting (dotted line), for the restoration of \texttt{FlyBrain} (left) and \texttt{Tube} (right).}
% \label{fig:acceler}
% \end{figure}
% \subsection{Application to real data}
% We finally test \textbf{BD3MG} in a real application problem with the same reconstruction task on data specifically acquired for the experiment. It consist in a 3D volume of mouse muscular tissue of size $400 \times 500 \times 100 $ pixels corresponding to a volume of $24,5\mu m \times 19,6\mu m \times 100\mu m$. The acquisition setting is the following:
% \begin{table}[ht]
%   \centering
%   \begin{tabular}{|c|c|} 
%     \hline
%     \textbf{Parameter} & \textbf{Setting} \\
%     \hline\hline
%     Support & Agarose gel \\
%     \hline
%     Excitation wavelength Ti & Sa (800nm)  \\
%     \hline
%     Mean laser power & 10mW on sample  \\
%     \hline
%     Exposure time & 2 \mu \text{s/pixel}   \\
%     \hline
%     PhotoMultiplier Tube 1 & 650V,Gain=3x,offset=32\% \\
%     \hline
%     PhotoMultiplier Tube 2 & 620V,Gain=3x,offset=20\% \\
%     \hline
%   \end{tabular}
%   \caption{Settings for the biphotonic microscopy acquisition of the volume \textit{mouse}}
%   \label{tab:setting}
% \end{table}
% Following the work of \cite{chouzenoux:hal-01985663}, we estimated gaussian point-spread function (PSF) within a 3D microscopic volume of mouse muscular tissue of size $400 \times 500 \times 100 $ pixels corresponding to a volume of $24,5\mu m \times 19,6\mu m \times 100\mu m$, by applying the \textbf{FIGARO} algorithm to photoreactive microbeads injected in the volume. To simplify the model and since microbeads injection is not homogeneous in the volume, the PSF is assumed to be only vertically dependant and constant on each horizontal plane, thus recquiring to fit one gaussian distribution per altitude. However, the distribution of microbeads being heterogeneous, the full blurring operator is completed on missing altitudes with linear interpolation of the parameters $(\sigma_{\mathsf{X}}(z),\sigma_{\mathsf{Y}}(z),\sigma_{\mathsf{Z}}(z),\varphi_{\mathsf{Y}}(z),\varphi_{\mathsf{Z}}(z))$ between next and previous PSF as described in figure \ref{fig:PSF}. Since no reconstruction score is available in this context, the regularization parameters $(\lambda,\delta,\kappa,\eta)$ are selected here by retrospective visual inspection. The reconstruction shown in figure \eqref{fig:reconstruction} demonstrates good contrastive and sharpness properties.
% \begin{figure}[ht]
% \centering
% \includegraphics[width=6cm]{PSF.png}
% %\vspace{-0.4cm}
% \caption{Kernel of estimated PSF along dimensions y and z for the 100 altitudes in the volume.}
% \label{fig:PSF}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=7cm]{Rawdata.png}
% %\vspace{-0.4cm}
%         \caption{Raw microscopic acquisition }
%         \label{fig:original}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=7cm]{Reconstructed.png}
%         \caption{Reconstruction }
%         \label{fig:reconstruction}
%     \end{subfigure}
    
%     \caption{Slice ($24,5\mu m \times 19,6\mu m$) at altitude z=50 of the original acquisition (\textit{left}) and after reconstruction (\textit{right}). The comparison shows that the definition of the muscular structure has been enhanced by the reconstruction.}
% \end{figure}
\section{Conclusion}\label{se:conclu}

In this paper, we have presented a new block distributed Majorize-Minimize Memory Gradient algorithm to tackle a wide class of large scale optimization problems. The main feature of our method lies in its distributed asynchronous formulation that allows for delays among workers, while theoretically maintaining the convergence guarantees and the practical performance of the powerful 3MG scheme. The new algorithm has been tested in the context of 3D image restoration under depth-variant blur. Experimental results underlined its scalability and efficiency\footnote{The code of BD3MG for depth-variant image deblurring has been made available at \texttt{https://github.com/mathieuchal/BD3MG}}. Future works will be focused on the extension to more general graph topologies.

